Revisiting Over-smoothing in Deep GCNs

Oversmoothing has been assumed to be the major cause of performance drop in deep graph convolutional networks (GCNs). In this paper, we propose a new view that deep GCNs can actually learn to anti-oversmooth during training. This work interprets a standard GCN architecture as layerwise integration of a Multi-layer Perceptron (MLP) and graph regularization. We analyze and conclude that before training, the final representation of a deep GCN does over-smooth, however, it learns anti-oversmoothing during training. Based on the conclusion, the paper further designs a cheap but effective trick to improve GCN training. We verify our conclusions and evaluate the trick on three citation networks and further provide insights on neighborhood aggregation in GCNs.

==> relatedworks.tex <==
\section{Related Works}
This is related works.
aaaaaaaaa
aaaaaaaaa

aaaaaaaaaaaa

aaaaaaaaaaaaaa

aaaaaaaaaaaaaa

aaaaaaaaaaaaa
